Federated Causal Discovery from Heterogeneous Data

Conventional causal discovery methods rely on centralized data, which is inconsistent with the decentralized nature of data in many real-world situations. This discrepancy has motivated the development of federated causal discovery (FCD) approaches. However, existing FCD methods may be limited by their potentially restrictive assumptions of identifiable functional causal models or homogeneous data distributions, narrowing their applicability in diverse scenarios. In this paper, we propose a novel FCD method attempting to accommodate arbitrary causal models and heterogeneous data. We first utilize a surrogate variable corresponding to the client index to account for the data heterogeneity across different clients. We then develop a federated conditional independence test (FCIT) for causal skeleton discovery and establish a federated independent change principle (FICP) to determine causal directions. These approaches involve constructing summary statistics as a proxy of the raw data to protect data privacy. Owing to the nonparametric properties, FCIT and FICP make no assumption about particular functional forms, thereby facilitating the handling of arbitrary causal models. We conduct extensive experiments on synthetic and real datasets to show the efficacy of our method. The code is available at https://github.com/lokali/FedCDH.git.

==> table_significance.tex <==

\begin{table}[h]
    \centering
    \begin{tabular}{ccccccccccccccc}
    \toprule[2pt]
    \multicolumn{3}{c}{Parameters}&\multicolumn{4}{c}{[FedCDH vs. FedPC]} & \multicolumn{4}{c}{[FedCDH vs. NOTEARS-ADMM]} & \multicolumn{4}{c}{[FedCDH vs. FedDAG]}\\
    \cmidrule(r){4-15}d &k &n&S-$F_1$&S-SHD&D-$F_1$&D-SHD&S-$F_1$&S-SHD&D-$F_1$&D-SHD&S-$F_1$&S-SHD&D-$F_1$&D-SHD \\
      % Dropout rate \%  & 0 & \multicolumn{2}{c}{10} & \multicolumn{2}{c}{30} &\multicolumn{2}{c}{50} & \multicolumn{2}{c}{70} & \multicolumn{2}{c}{90}  \\
      % \cmidrule(r){2-2}\cmidrule(r){3-4}\cmidrule(r){5-6}\cmidrule(r){7-8}\cmidrule(r){9-10}\cmidrule(r){11-12}Method & Full & Full & 0del& Full & 0del& Full & 0del& Full & 0del& Full & 0del \\
      \midrule[1pt]
   \textit{6} &10&100&0.00& \underline{0.05} & 0.01& 0.12&0.00& 0.01& \underline{0.11}& 0.10&0.00& 0.01& 0.01& 0.01\\
   \textit{12} &10&100&0.00& 0.01& 0.01& 0.01&0.00& 0.00& \underline{0.15}& 0.00&0.00& 0.00& \underline{0.11}& 0.00\\
   \textit{18} &10&100&0.00& 0.01& 0.00& 0.01&0.00& 0.00& 0.03& 0.00&0.00& 0.00& 0.02& 0.00\\
   \textit{24}&10&100&0.01& 0.01& 0.00& 0.01&0.00& 0.00& 0.01& 0.00&0.01& 0.01& 0.01& 0.00\\
   \textit{30}&10&100&0.00 &0.01& 0.00& 0.01&0.00&0.00&0.01& 0.00&0.00& 0.00& 0.00&0.00\\
   6 &\textit{2}&100&0.00& 0.00& 0.01& 0.01&0.01& 0.00& \underline{0.21}& 0.01&0.00& 0.00& 0.03& 0.00\\
   6 &\textit{4}&100&0.00& 0.01& 0.00& 0.01&0.01& 0.01& 0.01&0.00&0.00& 0.01& 0.01& 0.00\\
   6 &\textit{8}&100&0.00& 0.00& 0.01& 0.02&0.02& 0.01& 0.03& 0.02&0.00& 0.00& \underline{0.09}& 0.00\\
   6 &\textit{16}&100&0.00& 0.01& 0.01& 0.02&0.00&0.00& 0.10& 0.03&0.00& 0.00& \underline{0.07}& 0.00\\
   6 &\textit{32}&100&0.00& 0.00& 0.00& 0.00&0.00& 0.00& 0.04&0.01&0.00& 0.00& 0.03& 0.00\\
   6 &10&\textit{25}&0.00& 0.00& 0.01& 0.01&0.01& 0.01& \underline{0.26}& 0.02&0.00& 0.00& 0.03& 0.00\\
   6 &10&\textit{50}&0.00& 0.01& 0.01& 0.00&0.01& 0.00& \underline{0.99}& 0.03&0.00& 0.00& 0.02& 0.00\\
   % 6 &10&100&0.00& 0.00& 0.01& 0.02&0.00& 0.00& 0.99&0.03&0.00& 0.01& 0.03& 0.00\\
   6 &10&\textit{200}&0.00& 0.01& 0.01& 0.02&0.00& 0.00& 0.03& 0.02&0.00& 0.00& 0.11& 0.01\\
   6 &10&\textit{400}&0.00&0.01& 0.01& 0.01&0.01& 0.00& 0.03& 0.01&0.00& 0.01& 0.01& 0.00\\    
    \bottomrule[2pt]
    \end{tabular}
    \caption{For \textbf{Reviewer JTdu}: to show the statistical significance of our method compared with other baseline methods on the synthetic linear Gaussian model, we report the p values via Wilcoxon signed-rank test. For each baseline method, we evaluate four criteria: Skeleton $F_1$ (S-$F_1$), Skeleton SHD (S-SHD), Direction $F_1$ (D-$F_1$), and Direction SHD (D-SHD). We set the significance level to 0.05. Those p values higher then 0.05 are underlined. From the results, we can see that the improvements of our method are statistically significant at 5\% significance level.}
    \label{tab:my_label}
   \end{table}
